Mapping Out the HPC Dependency Chaos

High Performance Computing~(HPC) software stacks have become complex, with the dependencies of some applications numbering in the hundreds. Packaging, distributing, and administering software stacks of that scale is a complex undertaking anywhere. HPC systems deal with esoteric compilers, hardware, and a panoply of uncommon combinations. In this paper, we explore the mechanisms available for packaging software to find its own dependencies in the context of a taxonomy of software distribution, and discuss their benefits and pitfalls. We discuss workarounds for some common problems caused by using these composed stacks and introduce Shrinkwrap: A solution to producing binaries that directly load their dependencies from precise locations and in a precise order. Beyond simplifying the use of the binaries, this approach also speeds up loading as much as 7x for a large dynamically-linked MPI application in our evaluation.

==> text/background.tex <==
\section{Background}
\subsection{What's a Binary?}

The popularity of the \emph{bazaar} development model has resulted in an
explosion of software components. Using a 2018 post as a data point, there are
over 100 million open source repositories hosted on GitHub~\cite{100m-repos}
alone. The proliferation of packages, their dependencies among another and
compatibility across an ever increasing version matrix, has led to an emergence
of the curation of package groups through the creation of Linux distributions
and their associated tooling. There are currently over 300 actively maintained
Linux distributions and what delineates them are the composition of the
\emph{userland} binaries. In conjunction with the proliferation of packages, software itself has become
increasingly complex, as evidenced by the components necessary to run a binary
on Linux. The rising complexity of software and build tooling to reason on
sane software deployments models is a ongoing area of research.

In order to survey the distinction amongst Linux distributions and the means in
which they deliver and package software, comprehension of the final ultimate
target the application binary is a good place to start. What are the components
you need to run a binary in Linux? The entry point to a process is a file
following the \emph{Executable and Linkable Format (ELF)}, whose header
identifies various  metadata about the file itself such as endianness and must
be of the \emph{Executable File (EXEC)} type.

\begin{listing}[H]
\begin{minted}[fontsize=\small]{console}
$ readelf -h ruby
ELF Header:
  Magic:   7f 45 4c 46 02 01 01 ...
  Class:         ELF64
  Data:          2's complement, little endian
  Version:       1 (current)
  OS/ABI:        UNIX - System V
  ABI Version:   0
  Type:          EXEC (Executable file)
  Machine:       Advanced Micro Devices X86-64
\end{minted}
\caption{A sample ELF header for the Ruby interpreter using \emph{readelf} }
\end{listing}

Using language package dependencies as a proxy, software components may have a
median between 8 and 500 transitive dependencies\cite{forsgren20212020}
depending on the language. Some oggf these dependencies may be compiled into the file
statically. Additionally, the ELF format supports the resolution of dependencies
dynamically at invocation runtime through a process known as \emph{dynamic
linking} and are identified through the use of the \Verb`NEEDED` tag within
the \Verb`.dynamic` section of the file's header. Dynamic dependencies may also be
included at runtime through an invocation of \emph{dlopen}, functionality typically
offered through the standard C library to include dynamically shared objects.

Dependencies need not be constrained to code itself and as software complexity
has risen so too has it's configurability. Hence configuration files may become
a necessary, yet implicit, dependency for the execution of a binary. This
complexity has made it increasingly difficult to port software to new target
environments\cite{10.1145/3213846.3213855}.

\subsection{The Search for Dependencies}
The simplest deployment model for a software component is one restricted to a
\emph{single file}, statically linked. To support code reuse and allow for
security vulnerabilities to be transparently applied to a system at whole, it
has become common for binaries to rely on their dependencies dynamically through
\emph{dynamic linking}.

The shared objects required by a binary are encoded in a section within the ELF
header and loaded by the linker/interpreter at runtime. Each shared object may
itself require other needed libraries that are subsequently loaded until the
full transitive closure of needed libraries are made available.

\begin{listing}[H]
\begin{minted}{console}
$ patchelf --print-needed ruby
libruby-2.7.4.so.2.7
libz.so.1
libpthread.so.0
librt.so.1
libdl.so.2
libcrypt.so.1
libm.so.6
libc.so.6
\end{minted}
\caption{Transitive closure of shared objects needed by the Ruby interpreter }
\end{listing}

The instructions to the linker though on where to discover the required
dependencies are oftentimes implicit and there are a series of entrypoints for a
developer or sysadmin to exert control over the discovery mechanism. While there
are nuances in the exact search path order depending on how the dependencies are
listed in the file (i.e. if the dependency does not contain a slash), the order
can be simplified down to the following order: \Verb`RPATH`, \Verb`LD_LIBRARY_PATH`, \Verb`RUNPATH`, \Verb`/etc/ld.so.conf` and default system libraries (typically \Verb`/lib` or \Verb`/usr/lib`)\footnote{Building with the \Verb`-nodeflibs` flag will cause the linker to disregard these directories}. 

\begin{figure}[H]
    \includegraphics[width=\linewidth]{text/images/loading_order.png}
    \caption{The search order for the dynamic linker}
    \label{fig:loading_order}
\end{figure}

Typical binaries for many distributions do not use the explicit behavior of
\Verb`RPATH`, \Verb`LD_LIBRARY_PATH` or \Verb`RUNPATH` to direct the linker but rely on the default
system libraries or pre-seed the \Verb`ld.so.conf` file with the necessary
directories. The implicit search and well known directory paths are often
referred to as the \emph{Filesystem Hierarchy Standard~(FHS)}. The model assumes
a single namespace for all libraries and through implicit search paths allows
for transparent upgrades of dependencies. This is a constant point of contention
for systems that strive for reproducible and hermetic software deployments.

\subsection{Software Deployment Models}
The need to have sane software deployments have led to some non-traditional
Linux distributions and software models that work within the current
configurability offered by the dynamic linker. Potentially the simplest is the
ability for an application to refer to dynamic libraries within it's own
directory through the use of \Verb`$ORIGIN` when describing the path location
for the shared object. A novel approach gaining popularity are software
deployment models which are \emph{store-based}, where the central concept is a
read-only directory that contains all software components and uses a hashing
scheme in the name to distinguish different versions or variants of the same
software component. Dependencies for a software component may only refer to
other software components within the \emph{store}, forming an explicit directed
acyclic graph. The remaining software deployment models rely on a hermetic or
reproducible base root filesystem.


==> text/future.tex <==
\section{Challenges, Limitations and Future Work}\label{challenges}

% Shrinkwrap's current implementation has a few limitations imposed by the loader controls available.
% The design of the
% tool is meant to emboss dependencies of a desired shared object by lifting them
% to the needed section of the binary. By freezing the location of the
% dependencies the goal is to fix
% dynamic linking to the state it is in within the application's build environment.
% This approach works particularly well for store-based
% package managers where the absolute path includes a type of content addressable
% hash. The tool however could nevertheless be applied to binaries that resolve
% their dependencies via other mechanism, such as the FHS, and then there is no
% guarantee that the files will remain present or unmodified.
% 
% Attempting improvements very low in the stack proved challenging as there are
% very little tools to debug failures and little is written about the subject
% publicly. When modifying binaries, specifically the ELF header, a small
% innocuous coding error can easily result in a \Verb`Segmentation fault`. This
% failure can occur early enough during process startup that in fact it is during
% the execution of the interpreter or dynamic linker, which makes it difficult to
% apply well known debugging paradigms such as print-logging or using a debugger
% (gdb). While we encountered a plethora of libraries designed to read the ELF
% file format, few existed to modify the header and to do so correctly. We
% discovered the ELF header format to be simple in design but complicated it in
% it's use with many sections referencing each other that need to be correctly
% changed in tandem. Validating the correctness of code is always difficult.
% 
% Traditional Linux distributions typically have a
% caching mechanism as well via \Verb`/etc/ld.so.conf.cache` that would map the
% filename to its absolute path. This mechanism works well when the expectation
% is to only ever have a single file with the same basename. Unfortunately within
% store-like systems such as Spack, a single library name can exist multiple times
% within the store. Using the library name as the cache key no longer sufficed.
% The pattern of embossing the absolute paths on the binary is well suited to the
% store-model since the absolute paths themselves are considered read-only, and
% the dependency links between entries in the store are considered immutable.

The tools provided by the linker allow augmenting the search space for shared
objects in ways that were well-meant when done, in the mid-late 1990s, but that
have not aged well with time.  The behavior of RPATH was sufficiently reviled on
SunOS, Solaris and later on Linux that it has been deprecated for 20 years, mainly for misuse, yet
it's still supported and in active use in newly written systems to this day.
Its replacement, RUNPATH, was meant to solve all the worlds ills by ensuring
that LD\_LIBRARY\_PATH would still be usable, and that executables wouldn't
pollute their dependencies with their search path.  It succeeded in these goals,
but in preventing the RPATH from being used concurrently and eschewing propagation itself it completely lost the
ability to propagate search paths to dependencies when necessary.

In the end, the desired effects are generally a simpler combination of options
to inject new paths into the library search path:
\emph{prepend, append, and whether to inherit}. All of the problems listed in
Section~\ref{sec:issues} but one can be solved by offering prepend/append and a
flag to propagate or not on each path added to the search space.  

The desire to find all libraries within a few well-known directories from the
FHS model has bled into the ability to specify the search space as a single
list for all libraries. This can easily lead to cases where a library can
be found in unintended locations and a large search space can also impose a
meaningful performance impact as it must be searched in $\mathcal{O}(n)$ rather
than constant time. Although we've presented Shrinkwrap as a solution to this
problem, we could do better with deeper or more expressive interfaces to the loader. Allowing
the ability to dictate the search space per shared object would give fine
grained control over the search semantics.  This would also solve the final
issue, the ability to load libraries with conflicting filenames from paths
deterministically.

Having considered this direction, the other question that must be asked is why
we must rely on a bare soname and a linear set of paths to search to do this
job.  The fuschia kernel and zircon system loader actually implement a service
to request dynamic libraries at load time, allowing load configurations to be
changed between libraries during loading~\cite{fuschia-loading}.  In the end
though, there is a standard ELF loader on top of it.  Given the option to change
the way dependencies are encoded in binaries could allow a system like Nix or
Spack to store the hash of the library being requested, store the specification used to
build it, or otherwise enough information to be able to not just load it, but
determine with far greater detail which version is expected if it's not
available.  One can envision a system that would allow a user to take a binary
set up that way and ask a tool to provide all the dependencies it needs in place
of distributing a static binary or a container.

% Finally, changing the needed dynamic dependencies to point to absolute paths, especially when those paths are immutable and content-addressable, may have philosophical and legal considerations for certain open-source licenses such as \emph{LGPL}\cite{lgpl}. What specifically distinguishes a static binary to one dynamically loaded but with fixed dependencies? LGPL specifically mentions that only in the case of dynamic linking is the license not propagated over. 
% 
% \begin{quote}
%     \emph{1) Use a suitable shared library mechanism for linking with the Library. A suitable mechanism is one that (a) uses at run time a copy of the Library already present on the user's computer system, and (b) will operate properly with a modified version of the Library that is interface-compatible with the Linked Version.}
% \end{quote}
% 
% Although these dependencies go through the process of being dynamically linked, the library they are linked to is effectively fixed. Does this distinction blur the differentiation between static and dynamic linking? What if the linker validated the content-address to also verify the library hasn't been changed? Additional investigation into the legal ramifications may be an opportunity for future work.

==> text/todo.tex <==
\section{TODO}

